IsaBIL: A Framework for Verifying (In)correctness of Binaries in Isabelle/HOL (Extended Version)

This paper presents IsaBIL, a binary analysis framework in Isabelle/HOL that is based on the widely used Binary Analysis Platform (BAP). Specifically, in IsaBIL, we formalise BAP's intermediate language, called BIL and integrate it with Hoare logic (to enable proofs of correctness) as well as incorrectness logic (to enable proofs of incorrectness). IsaBIL inherits the full flexibility of BAP, allowing us to verify binaries for a wide range of languages (C, C++, Rust), toolchains (LLVM, Ghidra) and target architectures (x86, RISC-V), and can also be used when the source code for a binary is unavailable. To make verification tractable, we develop a number of big-step rules that combine BIL's existing small-step rules at different levels of abstraction to support reuse. We develop high-level reasoning rules for RISC-V instructions (our main target architecture) to further optimise verification. Additionally, we develop Isabelle proof tactics that exploit common patterns in C binaries for RISC-V to discharge large numbers of proof goals (often in the 100s) automatically. IsaBIL includes an Isabelle/ML based parser for BIL programs, allowing one to automatically generate the associated Isabelle/HOL program locale from a BAP output. Taken together, IsaBIL provides a highly flexible proof environment for program binaries. As examples, we prove correctness of key examples from the Joint Strike Fighter coding standards and the MITRE database.

==> sections/curl-double-free-OLD.tex <==


\section{Case Study: Double-Free Vulnerability in cURL (CVE-2016-8619)}
\label{sec:double-free-curl}

\begin{figure}
  \centering
  \begin{mdframed}[backgroundcolor=backcolour,hidealllines=true,%
                   innerleftmargin=0,innerrightmargin=0,
                   innertopmargin=-0.2cm,innerbottommargin=-0.2cm]
    \lstinputlisting[language=c,escapeinside={(*}{*)},lastline=11,basicstyle=\tt\fontsize{7}{7.5}\selectfont]{C/curl-vuln.c}
  \end{mdframed}
  \vspace{-1.7ex}
  \begin{mdframed}[backgroundcolor=red!10,hidealllines=true,%
                     innerleftmargin=0,innerrightmargin=0,
                     innertopmargin=-0.15cm,innerbottommargin=-0.12cm]
  \begin{minipage}{0.5\textwidth}
    \begin{mdframed}[backgroundcolor=red!10,hidealllines=true,%
                     innerleftmargin=0,innerrightmargin=0,
                     innertopmargin=-0.15cm,innerbottommargin=-0.12cm]
      \lstinputlisting[language=c,escapeinside={(*}{*)},backgroundcolor=\color{red!10},   
                       firstline=12,lastline=15,showlines=true,firstnumber=12,basicstyle=\tt\fontsize{7}{7.5}\selectfont]{C/curl-vuln.c}
    \end{mdframed}
  \end{minipage}
  \hfill
  \begin{minipage}{0.494\textwidth}
    \begin{mdframed}[backgroundcolor=green!10,hidealllines=true,%
                     innerleftmargin=0,innerrightmargin=0,
                     innertopmargin=-0.15cm,innerbottommargin=-0.12cm]
      \lstinputlisting[language=c,escapeinside={(*}{*)},backgroundcolor=\color{green!10},
                       firstline=12,firstnumber=12,lastline=15,numbers=none,basicstyle=\tt\fontsize{7}{7.5}\selectfont]{C/curl-sec.c}
    \end{mdframed}
  \end{minipage}
  \end{mdframed}
  \vspace{-1.7ex}
  \begin{mdframed}[backgroundcolor=backcolour,hidealllines=true,%
                   innerleftmargin=0,innerrightmargin=0,
                   innertopmargin=-0.2cm,innerbottommargin=-0.2cm]
    \lstinputlisting[language=c,escapeinside={(*}{*)},firstline=16,firstnumber=16,basicstyle=\tt\fontsize{7}{7.5}\selectfont]{C/curl-vuln.c}
  \end{mdframed}
  \vspace{-1ex}
  \caption{The \ReadData function of the cURL library in \code{security.c}.
           The snippet highlighted in \colorbox{red!10}{red} shows the vulnerable code in version 7.50.3, and that in \colorbox{green!10}{green} shows the corrected vulnerability in version 7.51.0.}
  \label{fig:curl-double-free}
\end{figure}



cURL is an open-source library primarily used for transferring data over the internet 
using various protocols, including TLS.
It has a large user base, supporting multiple operating systems and architectures (including \RiscV), and thus ensuring the security of cURL is critically important. 


Unfortunately, however, cURL has been known to contain vulnerabilities.
Consider the function \ReadData in \cref{fig:curl-double-free}, which underpins the Kerberos authentication protocol in cURL (prior to version 7.51.0), where 
% Explain
\cref{line:read-data-read-len} reads the length of an incoming 
data packet from a socket.
If this succeeds, \code{socket\_read} will return a 0, causing the if statement on 
\cref{line:read-data-result} to fall through.
Then, on \cref{line:read-data-ntohl} the call to \code{ntohl} converts 
the data length (\code{len}) from network byte order (big-endian) to host byte order (big- or little-endian). 
Note that this method does not sanitize its input.
Next, \Realloc on \cref{line:read-data-realloc} resizes the \code{data} buffer in \KrbBuffer, % using the length returned from the socket. \Realloc will return 
and returns 
either a new pointer to the resized memory, or \code{NULL} 
if an error occurs.
The rest of the method then reads and decodes the remaining data from the socket.

The caller is responsible for managing the \KrbBuffer pointer by allocating it before and freeing it after calling \ReadData.
Here we assume \Malloc is called directly before \ReadData
and free is called directly after, as follows:
\lstinline{malloc(buf, sz); read_data(conn, fd, buf); free(buf);}

If receiving data from the socket on \cref{line:read-data-read-len} yields a length of 0 ($\code{len}=0$), the call to \Realloc with $\code{len} = 0$ results in \emph{zero reallocation}, leading to \emph{undefined behaviour}\footnote{\url{https://www.open-std.org/jtc1/sc22/wg14/www/docs/n2464.pdf}}. %, which must be avoided.
Most implementations of \Realloc %on GLIBC, MSVC, zOS and AIX this 
will return NULL and free the pointer following a \emph{zero reallocation}.
%In BSD, NULL is returned only if there is not enough memory, the pointer is not freed and is returned without being changed.
As such, since the \KrbBuffer buffer is already freed before \Realloc returns and the caller is expected to free it after the function returns, this will lead to a \emph{double-free vulnerability}, identified by the vulnerability enumeration \href{https://cve.mitre.org/cgi-bin/cvename.cgi?name=2016-8619}{CVE-2016-8619}.

% This vulnerability arises due to undefined behaviour from zero-reallocations,
% which may lead to double free or other memory incorrectness vulnerabilities,
% and therefore should be avoided.

This vulnerability is resolved in version 7.51.0 of cURL by preempting the zero-allocation that leads to it: as highlighted in \colorbox{green!10}{green} in \cref{fig:curl-double-free}, placing a guard around the call to \Realloc \footnote{\url{https://github.com/curl/curl/commit/3d6460edeee21d7d790ec570d0887bed1f4366dd}} ensures that it is not called with a zero length. As such, if $\code{len}=0$, then the call to \Realloc is skipped,
\code{TMP} remains \code{NULL} and returns 0.
This ensures consistent behaviour across all C implementations.% \footnote{\url{https://github.com/curl/curl/blob/curl-7_50_3/lib/security.c}}.%#L190

\subsection{Scalability of the Parser}

\begin{figure}
  \centering
  \begin{mathpar} \footnotesize
  \inferrule[(\ReallocRule)]{
    \ReallocPredicate(\Command) \and
    w = \GetFreedAddr{\Command} \\\\ 
    sz = \GetSz{\Command} \\\\
    \MemoryTrace' = \MemoryTrace.[\AllocOp] }{ (\Command, \MopState)
    \ReallocSmallStep \MopStateE{\MemoryTrace'} } 
  \and 
  \inferrule[(\ZeroReallocRule)]{
    \ReallocPredicate(\Command) \and
    w = \GetFreedAddr{\Command} \\\\
    sz = \GetSz{\Command} \and
    sz = 0 \\\\
    \MemoryTrace' = \MemoryTrace.[\FreeOp] }{ (\Command, \MopState)
    \ReallocSmallStep \MopStateE{\MemoryTrace'} } 
    \and 
  \inferrule[(\SkipRule)]{
    \neg\FreePredicate{\Command} \\\\
    \neg\AllocPredicate{\Command} \\\\
    \neg\ReallocPredicate(\Command)
  }{ (\Command, \MopState)
    \ReallocSmallStep \MopState 
  }
  \end{mathpar}
  \vspace{-10pt}
  \caption{Reallocation semantics}
  \label{fig:reallocation-steps}
  \vspace{-10pt}
\end{figure}


We cross compile cURL \curlold and 7.51.0 for \RiscV on Linux using the GNU \RiscV compiler 
with the default options.
We modify the source code for \ReadData by adding the \lstinline{noinline} attribute, which ensures the function is not inlined.
Note that \lstinline{noinline} is not a requirement for verification, but facilitates compositional reasoning (see \cref{sec:curl-comp}). 


% Although the program in \cref{fig:curl-double-free} comprises fewer than 30 lines of code, 
Using the generated BIL directly creates a scalability challenge. 
% The associated assembly and BIL are much larger, posing a scalability challenge. In particular, 
The assembly corresponding to version 7.50.3 contains {\em 63,592 \RiscV instructions}, which equates to {\em 127,023 LoC in BIL} with {\em 63,592 BIL instructions} (the numbers for version \curlfixed are similar).
% These locales correspond to the binaries for cURL 7.50.3 and 7.51.0,
% auto-generated from their respective BIL programs.
%
Naively generating the corresponding \IsaBIL locales 
(see \cref{sec:parser}) takes approximately 14 minutes, which is impractical for verification. Of this, 
the lexer takes 4s, the parser takes 2s, and the translator takes approximately 13 minutes.
The wait time in the translator arises from instantiating the Isabelle/HOL locale
in the current proof context, an operation which cannot be avoided.

To address this, we extend the \CommandBILfile command with a \emph{new option}, \CommandwithSR, to focus only on the subroutines of interest (and their dependencies). For example, to generate the \IsaBIL locale for \code{read\_data} in version 7.50.3, we use the following command: 
\begin{lstlisting}[language=isabelle,escapeinside={(*}{*)},numbers=none,backgroundcolor=\color{white}]
    BIL_file (*\guilsinglleft*)libcurl.7.50.3.bil.adt(*\guilsinglright*) defining read_data_7_50_3
      with_subroutines read_data and ... 
\end{lstlisting}
where ``\dots'' contains functions that \ReadData calls (e.g., \code{ntohl}). 
% Where \code{libcurl.7.50.3.bil.adt} and \code{libcurl.7.51.0.bil.adt}
% are files containing the BIL for the bad and good programs in \cref{fig:curl-double-free}
% in \BILa format. \CurlBadLocale and \CurlGoodLocale is the name of the locale to be generated.
% The subroutines \code{Curl\_read\_plain}, \code{recv} and \code{\_\_bswapsi2} are
% called by \ReadData and thus are also needed for verification, noting 
% that the compiler has inlined or replaced any other function that may appear in \ReadData
% (i.e. \code{ntohl} = \code{\_\_bswapsi2}).
Running \CommandBILfile now takes only 6s, with 131 instructions to verify in version 7.50.3 and 132 instructions in version 7.51.0.

We next show how we detect this vulnerability in version 7.50.3 using an incorrectness proof, and prove the corrected code in version 7.51.0. 


% This wait time is impractical for the verification we aim to 
% accomplish in this example. 

% matching each \RiscV instruction.
% The assembly for 7.51.0 contains 63745 \RiscV instructions
% The BIL file totals 127392 lines, with 63745 BIL instructions matching each \RiscV instruction. 



\subsection{(In)correctness of the \ReadData Subroutine}
\label{sec:incorr-readd-subr}

% \paragraph{The \CurlBadLocale and \CurlGoodLocale locales}

% % This can be rectified by hiding symbols that are irrelevant for this extracting from the binary only the symbols necessary
% % for our verification.\bd{Make it clear which symbols are needed}
% Thus, our call to the BIL parser for the \ReadData functions looks like this:

% \begin{lstlisting}[language=isabelle,escapeinside={(*}{*)},numbers=none,backgroundcolor=\color{white}]
%     BIL_file (*\guilsinglleft*)libcurl.7.50.3.bil.adt(*\guilsinglright*) defining Lib_Curl_7_50_3
%       with_subroutines read_data and Curl_read_plain and recv and "__bswapsi2"
%     BIL_file (*\guilsinglleft*)libcurl.7.51.0.bil.adt(*\guilsinglright*) defining Lib_Curl_7_50_3
%       with_subroutines read_data and Curl_read_plain and recv and "__bswapsi2"
% \end{lstlisting}

% % \bd{Need to argue why this is OK}

As described above, \ReadData contains a double-free vulnerability. However, unlike our prior example (\cref{sec:double-free-paper}), the vulnerability arises from a reallocation of memory. Thus, we first describe the construction of a \ReallocLocale locale, which reuses our parts of the \AllocationLocale. Then, we prove both incorrectness of version \curlold, as well as correctness of \curlfixed of \ReadData.  


\paragraph{The \ReallocLocale locale}
% In the double-free proofs in \cref{sec:double-free-paper}, we introduced a 
% simple allocation model, instantiated for BIL and encoded in the \AllocationLocale locale.
% However, this model does not consider reallocations and thus we require
% a new allocation model capable of capturing calls to \Realloc.
%
We define \ReallocLocale by instantiating the small-step transition 
relation $\BilSmallStep$ of \Locale{BIL\_semantics} (see
\cref{sec:local-locale-1}).
Whilst we do not extend \AllocationLocale from \cref{sec:double-free-paper} directly, as it already defines small step 
semantics ($\AllocSmallStep$) that are incompatible with reallocation, we 
can borrow:
%
\begin{enumerate*}
  \item the definition of $\memop$,
  \item our abstract allocator $\NextAddrAllocatorName$,
  \item our memory trace $\MemoryTrace$,
  \item the getter for the size $\GetSzName$,
  \item the getter for the pointer to free $\GetFreedAddrName$,
  \item the predicate that denotes a program is freeing memory $\FreePredicateName$ and
  \item the predicate that denotes a program is allocating memory $\AllocPredicateName$.
\end{enumerate*}
%
These concepts are explained in detail in \cref{sec:double-free-paper}.

% In order to extend our allocation model to support reallocation, 
% we must understand the requirements for resizing allocated memory.
We use the predicate
$\ReallocPredicate$ to determine whether the 
next instruction to be executed in the given $\Command$
corresponds to a \Realloc instruction. We assume that an instruction that frees or allocates memory cannot simultaneously
perform an reallocation and vice versa, i.e.,
$\neg \FreePredicate{\Command} \lor 
 \neg \AllocPredicate{\Command} \lor 
 \neg \ReallocPredicate(\Command)$. 

When a program reallocates memory it has two parameters, 
a pointer to the memory to be resized, and the new size of that memory.
We utilise the existing functions $\GetSzName$ to obtain the 
size reallocated and 
$\GetFreedAddrName$ to obtain the address that
is reallocated. 
The size and location can be determined using the $\Decode$ function
on the given $\Command$.
The size and location are then used to add an $\AllocOp$ to the 
$\MemoryTrace$.
However, if the size of a reallocation is 0, this represents a zero-reallocation, and hence a $\FreeOp$ is added to the $\MemoryTrace$.
This results in a small-step transition relation, $\ReallocSmallStep$, 
over reallocations as given in \cref{fig:reallocation-steps}.     
Note that we retain the \AllocRule and \FreeRule rules 
from \cref{fig:allocation-steps}, and adapt the 
\SkipRule to encompass is reallocations.
% We encode our new allocation model supporting {\em reallocations} as the locale
% $\ReallocLocale$, fixing the functions \NextAddrAllocatorName,
% \FreePredicateName, \AllocPredicateName, \ReallocPredicate, \GetSzName and \GetFreedAddrName. 
% This locale is derived as an \emph{interpretation} of the locale $\BilInferenceLocale$
% retaining the decode predicate $\BILDecodeTransition$ and address set
% $\ProgramDomain$ as abstract, but overriding
% $\BilSmallStep\ =\ \AllocSmallStep$. Thus, we have the
Finally, we obtain the signature 
\[\ReallocLocale = (\BILDecodeTransition, \ProgramDomain,
  \NextAddrAllocatorName, \FreePredicateName, \AllocPredicateName, \ReallocPredicate,
  \GetSzName, \GetFreedAddrName)\] 
where the parameters $\NextAddrAllocatorName$, $\FreePredicateName$, $\ReallocPredicate$,
$\AllocPredicateName$, $\GetSzName$ and $\GetFreedAddrName$ are used to derive
$\ReallocSmallStep$ within the locale.


\paragraph{The {\tt read\_data} proof locales}
%
We combine the two locales generated for cURL binaries to produce
two new locales \CurlBadProofLocale and \CurlGoodProofLocale.
Reallocations are handled by calls to a PLT stub for \Realloc
so we can proceed in the same way as \code{malloc}/\code{free}.
In \cref{sec:double-free-paper}, we discussed how the first argument
of a subroutine call is stored in the register {\tt X10}.
Reallocations take two arguments:
\begin{enumerate*}
  \item a pointer to memory, and 
  \item a size.
\end{enumerate*}
The second argument (2) is stored in the return register ({\tt X11}),
thus 
% when fetching the size during a reallocation, we must instead 
% check this register.
% Therefore, 
we instantiate the parameters of \ReallocLocale as follows
for both locales:
\begin{align*}
  \ReallocPredicate{(\_,pc,\_)} &= (pc = \SymbolTable(``{\tt realloc}")) \\
  \GetSz{\Variables,pc,\_} &= 
    \begin{cases}
      \Variables({\tt X11}) & \textbf{if $pc = \SymbolTable(``{\tt realloc}")$} \\
      \Variables({\tt X10}) & \textbf{otherwise} 
    \end{cases}
\end{align*}

The remaining definitions of \GetFreedAddrName, \FreePredicateName
and \AllocPredicateName match that defined in \AllocatorLocale (\cref{sec:double-free-paper}).

\begin{theorem} 
\label{thm:curl-read-data-locale} 
Let $\ProgBad$ and $\ProgGood$ be the programs corresponding to \CurlBadLocale and
\CurlGoodLocale, respectively. Both of the following
hold
\begin{enumerate}[leftmargin=15pt]\small
  \item $\IncorrectnessProof{\neg \IsDF}{\ \ProgBad\ }{Q}{\IsDF}$
  \item $\HoareTriple{\neg \IsDF}{\ \ProgGood\ }{\neg \IsDF}$    
\end{enumerate}
\end{theorem}

% \cref{thm:curl-read-data-locale}, proven in Isabelle/HOL, establishes 
% the incorrectness and correctness of the example in \cref{fig:curl-double-free}.

% The incorrectness proof consists of X lines and Y lemmas, taking Z seconds to solve.
% The correctness proof consists of X lines and Y lemmas, taking Z seconds to solve.
% The correctness proof in \emph{(2)} of \cref{thm:curl-read-data-locale} requires 
% exploring all possible execution paths to ensure that there are no double free 
% vulnerabilities.
% Thus the proof is longer.


\subsection{Compositionality}
\label{sec:compositionality}
\label{sec:double-free-curl-compositional}
% This isn't enough for a full proof...
\label{sec:curl-comp}
\begin{figure}
  \centering
  \scalebox{0.9}{%
  \begin{tikzpicture}
    \node[rect] (ReadData) {\ReadData};
    \node[rect, right=2em of ReadData] (SecRecv) {\SecRecv};
    \node[rect, right=2em of SecRecv] (ChooseMech) {\code{choose\_mech}};
    \node[rect, fill=red!30, right=2em of ChooseMech] (CurlSecLogin) {\code{Curl\_sec\_login}};
    % \node[rect, right=2em of CurlSecLogin] (FtpStatemachAct) {\code{ftp\_statemach\_act}};
    % \node[rect, right=2em of FtpStatemachAct] (FtpConnect) {\code{ftp\_connect}};
    % \node[rect, dotted, fill=red, above right=0em and 2em of FtpConnect] (CurlHandlerFtp) {\code{Curl\_handler\_ftp}};
    % \node[rect, dotted, fill=red, below right=0em and 2em of FtpConnect] (CurlHandlerFtps) {\code{Curl\_handler\_ftps}};

    % \node[rect, below right=0em and 2em of CurlHandlerFtps] (AndMore) {\code{...}};

    \path[draw, thick, ->] (SecRecv) -- (ReadData); 
    \path[draw, thick, ->] (ChooseMech) -- (SecRecv); 
    \path[draw, thick, ->] (CurlSecLogin) -- (ChooseMech); 
    % \path[draw, thick, ->] (AndMore) -- (CurlHandlerFtp); 
    % \path[draw, thick, ->] (AndMore) -- (CurlHandlerFtps); 

    
  \end{tikzpicture}}%
  % \caption{The callgraph of functions in libcurl that call \ReadData.
  %          Entrypoints are coloured in red.
  %          Callbacks (which cannot directly be verified) are outlined with dotted lines.
  %          Note that this does not include other functions called as part of executing these methods.}
  \caption{A partial call graph in cURL demonstrating a path from an external function (\colorbox{red!30}{highlighted}), \code{Curl\_sec\_login}, to the internal function \ReadData.
           % Note that this does not include other functions called as part of executing these methods.
           }
  \label{fig:curl-callgraph}
\end{figure}


The proof in \cref{fig:curl-double-free} covers the \ReadData subroutine in the cURL library. 
However, this subroutine is an \emph{internal} function (i.e. not defined in a header file), making the vulnerability difficult to exploit directly in practice.
Nevertheless, as shown in the call graph in \cref{fig:curl-callgraph}, there is a path from an \emph{external} function (defined in a header file), namely \code{Curl\_sec\_login}, to \ReadData.
That is, a call to \code{Curl\_sec\_login} includes a call to \code{choose\_mech}, which in turn includes a call to \code{sec\_recv}, which itself calls \ReadData.
As such, the vulnerability in \ReadData \emph{could potentially} be exploited by a call to \code{Curl\_sec\_login}.  
% To see the bigger picture,  outlines a callgraph for libcurl indicating which functions call 
% \ReadData, and successively, which functions call the functions which call \ReadData.
% For example, \SecRecv calls \ReadData directly, and \code{choose\_recv} calls 
% \ReadData indirectly by calling \SecRecv.

% All of the functions which call \ReadData directly or indirectly are likely 
% to be susceptible to the same double free vulnerability.
Note that this may not always be the case, as freeing the data buffer pointer is left up to the caller, not the callee, and thus further incorrect behaviour to by caller (in this case a function above \ReadData in the call graph) could
rectify this vulnerability by forgetting to call free, or 
perhaps reallocating the pointer again before freeing it. 
Thus, we should aim to establish that each of these methods are (in)correct formally.

We do this in a \emph{compositional} fashion through \emph{proof reuse}: we reuse the (in)correctness specifications we prove at lower levels of the call graph in higher levels.
For instance, when proving that \code{sec\_recv} is (in)correct, we reuse the specification of \ReadData in \cref{thm:curl-read-data-locale} as a lemma. 
Indeed, this is precisely why we used the \code{noinline} attribute when compiling \ReadData: this allows us to reuse its specification; otherwise each call to \ReadData would be inlined, preventing us from proof reuse. 

% To motivate this argument, we now demonstrate how the proof for
% each of the functions in the tree are incorrect, using \SecRecv as an example.

% The higher we go in the call graph the more instructions we need to verify,
% and therefore the greater the proof burden, posing a scalability challenge.
% For example, \ReadData has X instructions, \SecRecv has Y instructions,
% and so on...
% This creates a scalability issue. 
%Our verification technique must therefore aim to address this somehow.


% First, we recall that from our introduction to big step semantics we can join proven triples 
% together using composition as follows:

% \begin{mathpar}
% \inferrule{
%   \OHearnTriple{R}{c'}{Q}
% }{
%   \OHearnTriple{P}{c}{Q}
% }
% +
% \inferrule{
% }{
%   \OHearnTriple{R}{c'}{Q}
% }
% =
% \inferrule{
%   \inferrule{
%   }{
%     \OHearnTriple{R}{c'}{Q}
%   }
% }{
%   \OHearnTriple{P}{c}{Q}
% }
% =
% \inferrule{
% }{
%   \OHearnTriple{P}{c}{Q}
% }
% \end{mathpar}

% In the past we have used this behaviour to define common behaviours in our
% binary that execute over multiple instructions to speed up verification
% (see \cref{sec:big-step-semantics}).
% We can apply the same technique on a larger scale to verified functions, 
% so that they can be discharged with a single rule application as well.
% We will now use a similar technique to solve \SecRecv. 

% In the last section we proved that \ReadData was incorrect, this proof 
% can be thought of as follows (note the variable state $\Delta$ is left abstract for brevity):

% \begin{mathpar} \footnotesize
% \inferrule{%*[left=FullProof]{
% \inferrule{%*[left=Malloc]{
% \inferrule{%*[left=ReadData]{
% \inferrule{%*[left=Free]{
% \inferrule{%*[top=ProgBigStepLast]{
%   \OHearnTriple{\inarrC{\lambda \MemoryTrace.\ \inarr{\MemoryTrace' = \MemoryTrace.\left[\inarrC{\AllocOp, \\ \FreeOp,\FreeOp}\right]  \\ {} \wedge\neg \IsDF(\MemoryTrace)}}}{(\Delta, \Word, var)}{Q}
% }{
%   \OHearnTriple{\inarrC{\lambda \MemoryTrace.\ \inarr{\MemoryTrace' = \MemoryTrace.[\AllocOp,\FreeOp] \\{} \wedge \neg \IsDF(\MemoryTrace)} }}{(\Delta,\SymbolTable[``free''],var)}{Q}
% }
% }{
%   \OHearnTriple{\inarrC{\lambda \MemoryTrace.\ \inarr{\MemoryTrace' = \MemoryTrace.[\AllocOp,\FreeOp] \\ {} \wedge \neg \IsDF(\MemoryTrace)}}}{(\Delta,just before free,var)}{Q}
% }
% }{
%   \OHearnTriple{\inarrC{\lambda \MemoryTrace.\ \inarr{\MemoryTrace' = \MemoryTrace.[\AllocOp,\FreeOp] \\ {} \wedge \neg \IsDF(\MemoryTrace)}}}{(\Delta,\SymbolTable[``read\_data''],var)}{Q}
% }
% }{
%   \OHearnTriple{\neg \IsDF}{(\Delta,\SymbolTable[``malloc''],var)}{Q}
% }
% }{
%   \OHearnTriple{\neg \IsDF}{(\Delta,just before malloc,var)}{Q}
% }
% \end{mathpar}


% Where: the subroutine read data resides at addresses 0x1c2c2-1c3ea in the binary. \bd{Is this important}

% The rule ReadData, which steps from the start of read data to the return address (which calls free)
% is a is effectively a big-step triple for (in)correctness.
% The proof for 
%  To solve Y, we prove as we did in the last section a triple.
% at some point we hit \ReadData.
% Now, instead of proving \ReadData again, we can apply the big step.
% As a proof this looks like the following:

% Where: the subroutine sec recv resides at addresses 0x1c2c2-1c3ea in the binary.
% and at 0x1c388 we sec recv calls read data.
% and the subroutine sec recv resides at address 0x1c2c2 in the binary.

% This means that we only have to solve sec\_recv\_pre, sec\_recv\_post,
% and our new calls to free and malloc.
% Once we have are triple we solve the proof as we did before.

% \begin{lstlisting}[language=isabelle,escapeinside={(*}{*)}]
% BIL_file (*\guilsinglleft*)libcurl.7.50.3.bil.adt(*\guilsinglright*)
%   defining Lib_Curl_7_50_3
%   with_subroutines read_data and Curl_read_plain and recv and "__bswapsi2" and
%                    sec_recv and read    
% \end{lstlisting}

\newcommand{\SecRecvBad}{{\it SR}_{7.50.3}}
\newcommand{\ChooseMechBad}{{\it CM}_{7.50.3}}
\newcommand{\CurlSecLoginBad}{{\it CSL}_{7.50.3}}

In \cref{thm:sec-rev-vuln} below, we prove incorrectness specifications for the $\SecRecvBad$, $\ChooseMechBad$ and $\CurlSecLoginBad$ functions, showing that each of these functions do indeed exhibit a double-free vulnerability. 
Our proof is compositional in that the proof for each function reuses the specification of the function below it, as discussed above (e.g. the proof of $\SecRecvBad$ reuses the incorrectness specification of \ReadData in \cref{thm:curl-read-data-locale} as a lemma). 

\begin{theorem}
\label{thm:sec-rev-vuln}
Let $C \in \{\SecRecvBad, \ChooseMechBad, \CurlSecLoginBad\}$, be a program corresponding to the \curlold versions of \code{sec\_recv}, \code{choose\_mech} and \code{Curl\_sec\_login}. Then: 

$\IncorrectnessProof{\neg \IsDF}{\ C\ }{Q}{\IsDF}$. 

% \begin{enumerate}[leftmargin=15pt]\small
% \item 
% % \item $\IncorrectnessProof{\neg \IsDF}{\ \ChooseMechBad\ }{Q}{\IsDF}$. 
% % \item $\IncorrectnessProof{\neg \IsDF}{\ \CurlSecLoginBad\ }{Q}{\IsDF}$. 
% \end{enumerate}
% \bd{Matt to delete the bits that haven't been proved}

% \begin{enumerate}[leftmargin=15pt]
%   \item 
%   \item $\HoareTriple{\neg \IsDF}{\ \ProgGood\ }{\neg \IsDF}$    
% \end{enumerate}



% [\SecRecv is vulnerable to double free]
%     TODO
\end{theorem}

\cref{thm:sec-rev-vuln} demonstrates a scalable proof for the incorrectness specifications of the functions in \cref{fig:curl-callgraph}. 
% proof for \ReadData.  and makes use of the (compositional) big-step semantics offered by BIL's (in)correctness logic. 
We can apply similar techniques to verify their corresponding correctness specifications; we have elided these proofs as they are similar. 

% The remaining functions in \cref{fig:curl-callgraph} may be proved in the same way.

% Note that each big step lemma we solve can be increased further by encorporating this rule as an to the automated solver.


% A scalable proof of correctness proceeds in much the same way, however,
% will take much longer as every execution path must be explored.


% %Points to highlight: 
% %+ Pulse has FPs in case of black-box code


% Recall that we used the \code{noinline} attribute when compilining \ReadData, as otherwise each call to \ReadData would be inlined, preventing us from \emph{reusing} the (in)correctness specification we proved in \cref{}.s
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/double-free.tex <==

\subsection{Double Free}
\label{sec:double-free}

We now look to prove our first example, CWE-415: Double Free outlined
in \cref{sec:overview-and-motivation}. To classify this vulnerability,
we require a memory allocation model, which is not part of the BIL
semantics (\cref{sec:specification-of-bil}). Memory allocation in C is
reflected as a PLT stub in the binary and could have many different
implementations~\cite{DBLP:journals/pacmpl/MemarianGDKRWS19,DBLP:journals/jar/LeroyB08}
and is specific to the compiler and target architecture. For the
purposes of the Double Free example, because we are not analysing
correctness of the allocation implementation itself, we can leave
these details abstract.
% . If we were then we could look at
% the specific implemenation details.
In particular, we are only required to track the pointer (memory
address) that is allocated (and later freed). Similarly, the size of
the memory that is allocated is also not relevant, and is therefore
not tracked. To this end, we develop a locale, \AllocatorLocale,
that extends the BIL semantics (see \cref{fig:proofs}) with an abstract allocation model inspired by earlier works~\cite{DBLP:journals/pacmpl/MemarianGDKRWS19,DBLP:journals/jar/LeroyB08}. 


% We therefore use a more abstract allocation model via an allocation locale. That abstracts the low-level malloc implementation. For example, even with the double-free example, the PLT stubs for RISC-V and x86 are different, but can be abstracted by the same locale. 




\paragraph{The \AllocatorLocale locale} % We use a memory allocation
% model developed by , which comprises
% four operations \AllocOpName, \FreeOpName, \LoadOpName and
% \StoreOpName. For the purpose of the Double Free example, we can elide
% the details of the \LoadOpName and \StoreOpName operations since they
% are not used.
% \BIL's memory model is straightforward and is
% characterised by a linear sequence of assignments. 
% We simplify the
% memory allocation process by eliminating sized blocks of memory, and
% using fixed-size addresses, instead. With this in mind, w
We define \AllocatorLocale by instantiating the small-step
transition relation $\BILSmallStep$ of \BilLocale (see
\cref{sec:local-locale-1}). We start by defining two memory
operations:
\[
  \memop ::= \AllocOp \mid \FreeOp
\]
where $w$ is the memory being allocated or freed and $sz$ is the size. Additionally, we
assume an abstract allocation function
$\NextAddrAllocatorName : \memop^* \rightarrow word$ that serves the
purpose of selecting suitable memory addresses for allocation and
retrieves the next address from the allocator based on the given
history (sequence) of allocations and deallocations. For each
allocation, we use $\NextAddrAllocatorName$ to obtain the next
available memory address. Consequently, in the state of
\AllocatorLocale, we must track the sequence of $\memop$
operations, which is provided to $\NextAddrAllocatorName$ as an input
whenever an allocation occurs. For the Double Free example, no other
variables need to be tracked, hence we simply assume the state to be
this sequence, which we denote % variables are needed
% We denote this sequence by trace of memory operations as a sequence,
% denoted
$\MemoryTrace : \memop^*$.
% We refer to the allocator's state as $\Allocator$ with the
% operations $\UpdateAllocator$ and $\NextAddrAllocator$, which update
% the allocator's state and retrieve the allocator's next address
% respectively.  Therefore, we define the verification state to be the
% memory operation trace ($\poststate : \MopState$) We therefore
% define the type of the verification state to be a tuple, of the form
% $s : (\MemoryTrace, \Allocator)$.

Recall that by using the $\Decode$ predicate
(\cref{section:instr-semantics}), the BIL instruction corresponding to
$\Command = \BILMachineStateE{\Variables}{pc}{mem}$ can be uniquely
identified. We use predicates
$\FreePredicateName : prog \rightarrow bool$ and
$\AllocPredicateName : prog \rightarrow bool$, which hold when the
next instruction to be executed in the given $\Command \in prog$
corresponds to a free and allocation instruction, respectively.
% to identify a program state
% $\BILMachineStateE{\Variables}{pc}{mem}$, which either frees or
% allocates memory respectively.
We assume that an instruction that frees memory cannot simultaneously
perform an allocation and vice versa, i.e.,
$\neg \FreePredicate{\Command} \lor \neg
\AllocPredicate{\Command}$. 
When the instruction for $\Command$ is an allocation, 
we utilise the function
$\GetSzName: prog \rightarrow sz$ to obtain the size allocated and
when the instruction for $\Command$ is a
deallocation, we utilise the function
$\GetFreedAddrName: prog \rightarrow word$ to obtain the address that
is freed. The size and location can be determined using the $\Decode$ function
on the given $\Command$.
Thus, % a transition of the verification state
% $\MopState$ can be made with the step predicate
we define a small-step transition relation, $\AllocSmallStep$, over
allocations as follows:
\begin{mathpar}
  \inferrule[(\sc alloc)]{
    \AllocPredicate{\Command} \\\\
    w = \NextAddrAllocator \and sz = \GetSz{\Command} \\\\
    \MemoryTrace' = \MemoryTrace.[\AllocOp] }{ (\Command, \MopState)
    \AllocSmallStep \MopStateE{\MemoryTrace'} } 
\and 
\inferrule[(\sc free)]{
    \FreePredicate{\Command} \\\\
    w = \GetFreedAddr{\Command} \\\\
    \MemoryTrace' = \MemoryTrace.[\FreeOp] }{ (\Command, \MopState)
    \AllocSmallStep \MopStateE{\MemoryTrace'} } 
\and 
\inferrule[(\sc skip)]{
  \neg\FreePredicate{\Command} \\\\
  \neg\AllocPredicate{\Command} }{ (\Command, \MopState)
  \AllocSmallStep \MopState }
\end{mathpar}

We encode this {\em allocation model} as the locale
$\AllocatorLocale$, fixing the functions \NextAddrAllocatorName,
\FreePredicateName, \AllocPredicateName, \GetSzName and \GetFreedAddrName. This
locale is derived as an \emph{interpretation} of $\BilInferenceLocale$
retaining the decode predicate $\BILDecodeTransition$ and address set
$\ProgramDomain$ as abstract, but overridding
$\BilSmallStep\ =\ \AllocSmallStep$. Thus, we have the following
signature
\[
  \AllocatorLocale = (\BILDecodeTransition, \ProgramDomain,
  \NextAddrAllocatorName, \FreePredicateName, \AllocPredicateName,
  \GetSzName, \GetFreedAddrName)
\]
where the parameters $\NextAddrAllocatorName$, $\FreePredicateName$,
$\AllocPredicateName$, $\GetSzName$ and $\GetFreedAddrName$ are used to derive
$\AllocSmallStep$ within the locale.

% In order to leave the allocator operations abstract, we must fix
% $\NextAddrAllocatorName$. Furthermore, we fix the predicates
% $\FreePredicateName$, $\AllocPredicateName$ and
% $\GetFreedAddr{prog}$ which may be instantiated differently based
% upon the binaries granularity, language or compiler.



\paragraph{The \DoubleFreeBadLocale and \DoubleFreeGoodLocale
  locales} These locales correspond to the double free program % and
% their proofs of (in)correctness. We provide two instances of each
% corresponding to the bad and good examples. The locales corresponding
% to the program, i.e., \DoubleFreeBadLocale and
% \DoubleFreeGoodLocale 
and are {\em auto-generated} from the corresponding BIL programs
(shown in \cref{DF-bad-bil,DF-good-bil}). This step is trivial when
using \isabil's \lstinline[language=isabellen]{BIL_file} command,
which we have developed using Isabelle/ML. In particular, we simply
invoke the Isabelle/HOL commands:

\medskip
\qquad\qquad    \lstinline[language=isabellen]{BIL_file double_free_bad "double-free-bad.bil.adt"}

\qquad\qquad\lstinline[language=isabellen]{BIL_file double_free_good "double-free-good.bil.adt"}
    
\medskip 
\noindent where {\tt double-free-bad.bil.adt} is a file containing the
BIL for \autoref{DF-bad} in \BILa format and {\tt double\_free\_bad}
is the name of the locale to be generated. The good version is
similar.

% two locales \DoubleFreeGoodLocale and
% \DoubleFreeBadLocale for the good and bad versions of the double
% free example.

\paragraph{The \DoubleFreeProofLocale locales}
We combine the two locales generated from the BIL programs with our
allocator locale ($\AllocatorLocale$) to produce a two new locales
\DoubleFreeBadProofLocale and
\DoubleFreeGoodProofLocale. Recall from
\cref{sec:program-specification} that for each locale generated from a
\BILa program, we have access to a symbol table {\tt sym\_table}
mapping strings (i.e., external function calls) to the program address
at which the symbol appears. Note that when a BIL program calls a
function, it typically stores the return address, then jumps to the
function. The symbol corresponding to the program counter after the
jump contains the name of the external function, which is stored in
the symbol table. In RISC-V convention, the first argument of a
function call is stored in the register {\tt X10}. To allocate memory, 
function {\tt malloc} is called with the size as the first argument 
whereas to deallocate a pointer, function {\tt free} is called with 
the pointer as the first argument. Therefore, we can obtain the size 
allocated by a call to {\tt malloc} and pointer freed by a call to 
{\tt free} by retrieving the value stored in register~{\tt X10}.

% , which extends
% $\DoubleFreeBadLocale$ and inherits
% $\DoubleFreeBadLocale$. $\DoubleFreeProofLocale$ interprets
% $\AllocatorLocale$

We therefore instantiate the predicates $\FreePredicateName$,
$\AllocPredicateName$, $\GetSzName$ and $\GetFreedAddrName$ from the
\AllocatorLocale locale as follows:
\begin{align*}
  % \NextAddrAllocatorName           &= \text{remains abstract} \\
  \FreePredicate{(\_,pc,\_)}         &= (pc = \SymbolTable(``{\tt free}")) \\
  \AllocPredicate{(\_,pc,\_)}        &= (pc = \SymbolTable(``{\tt malloc}")) \\
  \GetFreedAddr{(\Variables,\_,\_)}  &= \Variables({\tt X10}) \\
  \GetSz{(\Variables,\_,\_)}         &= \Variables({\tt X10})
\end{align*}

The exact implementation of {\tt next\_free} occurs at a lower level
of abstraction, and depends on the allocation model. At this level, we
provide the main requirement axiomatically, i.e., we require
\[
  w = \NextAddrAllocator \implies (\forall i.\ \MemoryTrace(i) = \AllocOp \implies \exists j.\ j > i \wedge \MemoryTrace(i) = \FreeOp)
\]

This presents us with all the components necessary to prove
(in)correctness of our examples. The following predicate captures the
double-free over the memory state defined above:
\begin{align*}
    \IsDF 
   & = \lambda \MemoryTrace.\ 
      \exists i,j,w.\ \inarr{
      i < j \wedge \MemoryTrace[i] = \FreeOp \wedge \MemoryTrace[j] = \FreeOp \wedge {}   \\
  (\forall k.\  i <  k < j \implies \MemoryTrace[k] \neq \AllocOp)}
\end{align*}
Note that the predicate captures {\em only} the double-free
vulnerability and does not formalise other pointer misuse
vulnerabilties, e.g., use-after-free or free-before-alloc.
% \bd{say this isn't about pointer-misuse}


\begin{theorem} \label{thy:double-free} Let $\Command_{bad}$ and $\Command_{good}$ be the
  programs corresponding to \DoubleFreeBadLocale and
  \DoubleFreeGoodLocale, respectively.  Both of the following
  hold
  \begin{enumerate}[leftmargin=15pt]
  \item $\IncorrectnessProof{\neg \IsDF}{\ \Command_{bad}\ }{Q}{\IsDF}$
    
    
  \item $\HoareTriple{\neg \IsDF}{% \BILMachineStateE{\Variables_{DF}}{\SymbolTable[\text{``good"}]}{mem}
\ \Command_{good}\ }{\neg \IsDF}$    
\end{enumerate}
\end{theorem}

The proof for \cref{thy:double-free} requires the repeated application 
of O'Hearn and Hoare step lemmas described in \cref{sec:local-locale-1} 
until the program terminates. Execution of common patterns such as the 
external calls to {\tt free} and {\tt malloc} can quickly be discharged 
according to the optimisations described in \cref{sec:riscv-optimisations}. 
Deconstructing the BIL program step for each O'Hearn or Hoare step is 
totally automated for double free through the {\tt solve\_prog} Eisbach 
methods. This shows that the \autoref{DF-bad} contains the CWE-415: Double-Free
vulnerability, which but \autoref{DF-good} does not. Although both the
presence and absence of a double-free vulnerability is ``obvious'' at
the level of the C program, our analysis has been conducted entirely
at the level of the binary. The analysis also does not rely on the C
program source, thus could be applied to inspect programs of unknown
origin.

==> sections/proofs.tex <==
\section{Proofs}
\label{sec:proofs}
% \xES{I've highlighted a lot of the x86 in green as I'm not sure we'll have enough time to include it now}
% mention the nontrivial and implies proof

In this section, we discuss correctness and incorrectness proofs for a
handful of examples. We fix the target operating system to Ubuntu
22.04.2 LTS, the architecture to RISC-V and the compiler to the RISC-V
GNU toolchain 12.2.0 (g2ee5e430018) cross-compiler. To generate the
BIL files we use a pre-release of BAP (511b64c). The proofs for our
running double-free example are given in \cref{sec:double-free} and
the set of JSF examples in \cref{sec:forbidden-symbols}.
 
% For code compilation, we target . For RISC-V, we use
% . \xES{For x86 we use GCC 11.3.0}. , for our proofs we use the Isabelle/HOL
% 2022 release.

% \begin{table}[t]
%   \centering
%   \begin{tabular}[t]{l|l|l}
%     Examples & RISC-V & x86 
%     \\
%     \hline
%     AV Rule 17 & \xmark & ---
%     \\\input{sections/related-work}
%     AV Rule 19 & \xmark & ---
%     \\
%     AV Rule 20 & \xmark & ---
%     \\
%     AV Rule 21 & \xmark & --- % ()
%     \\
%     AV Rule 22  & \xmark & --- % (11, 12 almost done)
%     \\
%     AV Rule 23  & \xmark & --- % (11, 12 almost done)
%     \\
%     AV Rule 24  & \xmark & --- % (11, 12 almost done)
%     \\
%     AV Rule 25  & \xmark & --- % (11, 12 almost done)
%     \\
%     Double Free (good)  & \cmark & \cmark % (11, 12 almost done)
%     \\
%     Double Free (bad)  & \xmark & \xmark % (11, 12 almost done)
%   \end{tabular}
%   \caption{\xmark\ indicates examples proved vulnerable; \cmark\ 
%     indicates examples proved secure; example refer
%     to~\cite{BAP-TOOLKIT}} \mg{might be worth combining the two tables}
% \label{tab:results}
% \end{table}

\subsection{Workflow for double free}

Details of the proofs are available in \cref{sec:furth-deta-example}. 


\subsection{Additional examples: Joint Strike Fighter (JSF) Air Vehicle (AV) Examples}
\label{sec:forbidden-symbols}




\begin{table}[t] \footnotesize
\begin{minipage}[b]{0.44\columnwidth}
    \begin{tabular}{|@{~}l|l@{\ }|}
\hline
\textbf{Component}                      & \textbf{Lemmas} \\ \hline
Correctness                             & 13              \\ \hline
Incorrectness                           & 3               \\ \hline
Inference Rules                         & 2               \\ \hline
% IMP Validation                          & 2               \\ \hline
BIL Specification                       & 594             \\ \hline
BIL Inference                           & 13              \\ \hline
RISC-V optimisations                    & 74              \\ \hline
Alloc Model                             & 6               \\ \hline
Find Symbol                             & 0               \\ \hline
Double Free (total for both examples)   & 77              \\ \hline
AV Rules (total for all seven examples) & 187             \\ \hline
\end{tabular}
\caption{Overview of theories and lemma for each of \isabil's components.}
\label{tab:development-overview}
\end{minipage}
\hfill
\begin{minipage}[b]{0.54\columnwidth}
\begin{tabular}{|@{~}l|p{0.85\columnwidth}@{~}|}
  \hline
  \textbf{AVR} & \textbf{Description (the following shall not be used)}                                                                                               \\ \hline
  17               & The error indicator errno % shall not be used                                      
  \\ \hline
  19               & {\tt \textless{}locale.h\textgreater} and the setlocale function\footnotemark 
  %shall not be used
  \\ \hline
  20               & The {\tt setjmp} macro and the {\tt longjmp} functions
  % shall not be used                 
  \\ \hline
  21               & The signal handling facilities of {\tt \textless{}signal.h\textgreater} 
  %shall not be used               
  \\ \hline
  23               & The library functions {\tt atof}, {\tt atoi} and {\tt atol} from library {\tt \textless{}stdlib.h\textgreater} 
  %shall not be used            
  \\ \hline
  24               & The library functions {\tt abort}, {\tt exit}, {\tt getenv} and system from library {\tt \textless{}stdlib.h\textgreater} 
  % shall not be used 
  \\ \hline
  25               & The time handling functions of library {\tt \textless{}time.h\textgreater} 
  % shall not be used                 
  \\ \hline
\end{tabular} \smallskip


\caption{AV rules with description}
\label{tab:av-rules}
\end{minipage}
\vspace{-10pt}
\end{table}
% Do we additionally describe other incorrectness proofs?


\footnotetext{Of course {\tt \textless{}locale.h\textgreater}
  refers to the {\tt C} locale library and not the Isabelle locales
  used by \isabil.}

\paragraph{The \AvRuleLocale locale}
\bd{some intro text to explain the table - reference to Appendix C}
We refer to the AV Rule locales collectively using
\AvRuleLocale, where \Locale{*} represents the rule number.  For each
of the examples in \autoref{tab:av-rules} we auto-generate a
corresponding locale using the Isabelle command:
\begin{center}
\lstinline[language=isabellen]{BIL_file Av_Rule_* "av-rule-*.bil.adt"}
\end{center}
where {\tt av-rule-*.bil.adt} refers to a file % containing the BIL
for
each example in \autoref{tab:av-rules} in \BILa format.  




% by returning from the function after freeing the pointer {\tt p} as
% shown in \autoref{DF-good}. In this instance, we can prove that the
% program is correct. Our initial program state is similar to that used
% for incorrectness, we keep the register state the same but set our
% program counter to the address of the {\tt good} function. Moreover,
% we start in a pre-state satisfying \IsDF but, as this is a proof
% of correctness, aim to show that we finish in a post-state satisfying
% \IsDF. Therefore, the triple we prove takes the form:





% % \[
% % \forall i,w.\ (\MemoryTrace[i] = \FreeOp) \implies \forall j > i.\ \MemoryTrace[j] = (\FreeOp) \implies \exists k < i\ \wedge\ k > j.\ \MemoryTrace[k] = \AllocOp
% % \]

% % A proof of incorrectness for double free requires us to find the existence of some post-state where deallocations {\em exceed} allocations for a given memory pointer. It is not sufficient to {\em balance}  We characterize a post-state in which this behaviour has occured using the predicate \IsDF which holds iff $\forall w.\ \MemoryTrace[w] = 0$. Trivially

% % start in a valid pre-state and

% % . We  . We aim to show that the post state satisfies $IsntBalanced$

% Recall from \cref{sec:incorrectness} that proofs of incorrectness take the form $\IncorrectnessProof{P}{c}{Q'}{Q}$. 





% \mg{it is trivial to show that these programs are deterministic so we can reuse etc...}. To show correctness, we do not need to satisfy the same non-trivial requirements as incorrectness. As such, our proof is complete.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

